Mean Field Limits for Stochastic, Underdamped Reactive Langevin Dynamics Models

We rigorously derive the effective large-population, mean-field dynamics of particle-based reactive Langevin dynamics (PBRLD) models. These models extend particle-based stochastic reaction-diffusion (PBSRD) descriptions by incorporating velocities, inertial effects, and underdamped motion. In Isaacson, Liu, Spiliopoulos, and Yao, SIAP 2026, PBRLD models were formulated and shown to recover Doi volume reactivity PBSRD model in the overdamped limit. In this work we prove convergence of the associated measure-valued stochastic processes, representing species concentration fields on position-velocity phase space, to a deterministic mean-field limit. The limiting equations form a novel system of nonlocal kinetic reaction-diffusion partial integro-differential equations, coupling hypoelliptic transport with reaction terms that retain the spatial and velocity structure of the underlying particle interactions.

==> my_commands.tex <==
\usepackage{bbm}


% New commands:
\renewcommand{\vec}[1]{\boldsymbol{#1}}
\newcommand{\vecs}[1]{\boldsymbol{#1}}
% \renewcommand{\vec}[1]{\mbox{\boldmath${\rm #1}$}}
\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\brac}[1]{\left[#1\right]}
%\newcommand{\avg}[1]{\left<#1\right>}
\newcommand{\E}{\mathbb{E}}
\newcommand{\avg}[1]{\E\left[#1\right]}
\newcommand{\from}{\leftarrow}
\newcommand{\D}[2]{\frac{d#1}{d#2}}
\newcommand{\PD}[2]{\frac{\partial#1}{\partial#2}}
\newcommand{\PDD}[2]{\frac{\partial^{2}{#1}}{\partial{#2}^{2}}}
\newcommand{\PDDM}[3]{\frac{\partial^{2}{#1}}{\partial{#2}\partial{#3}}}
\newcommand{\PDN}[3]{\frac{\partial^{#1}{#2}}{\partial{#3}^{#1}}}
\newcommand{\pd}[2]{\partial_{#2}#1}
\newcommand{\lap}[1]{\Delta#1}
\newcommand{\lapd}[2]{\Delta_{#1}#2}
\newcommand{\at}[2]{\left.#1\right|_{#2}}
\renewcommand{\div}[1]{\nabla\cdot\vec{#1}}
%\newcommand{\grad}[1]{\nabla#1}
\newcommand{\dotV}[2]{\vec{#1}\cdot\vec{#2}}
\newcommand{\dotNV}[2]{#1\cdot#2}
\newcommand{\dx}{\Delta x\xspace}
\newcommand{\dt}{\Delta t\xspace}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\norm}[1]{\Vert#1\Vert}
\newcommand{\inprod}[1]{\left<#1\right>}
\renewcommand{\complement}{\mathbf{c}}
\newcommand{\beqparen}[1]{\big(#1\big)}
\newcommand{\eqparen}[1]{(#1)}
\newcommand{\sump}{\sideset{}{'}{\sum}}
\DeclareMathOperator{\erfc}{erfc}
\DeclareMathOperator{\prob}{Pr}
%\newcommand{\comment}[1]{{\color{blue}{\bf{#1}}}}
\newcommand{\Tmax}{T_{\textrm{max}}}
\newcommand{\kb}{k_{\text{B}}}
%\newcommand{\pl}{p_{\lambda}}
\newcommand{\Gl}{G_{\lambda}}
\newcommand{\dom}{\mathcal{D}}
\DeclareMathOperator{\diam}{diam}
\newcommand{\psibar}{\bar{\Psi}} 


\newcommand{\DA}{D_{\textrm{A}}}
\newcommand{\DB}{D_{\textrm{B}}}
\newcommand{\DC}{D_{\textrm{C}}}

% vector short cuts:
\newcommand{\br}{\vec{r}}
\newcommand{\bro}{\vec{r}_{0}}
\newcommand{\brb}{\vec{r}_{\rm{b}}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\khat}{\hat{k}}
\newcommand{\bi}{\vec{i}}
\newcommand{\bj}{\vec{j}}
\newcommand{\bk}{\vec{k}}
\newcommand{\bja}{\bj^{a}}
\newcommand{\bjb}{\bj^{b}}
\newcommand{\bjc}{\bj^{c}}
\newcommand{\bI}{\vec{I}}
\newcommand{\bJ}{\vec{J}}
\newcommand{\ve}{\vec{e}}
\newcommand{\ek}{\ve_{k}}
\newcommand{\vnu}{\vecs{\nu}}
\newcommand{\veta}{\vecs{\eta}}
\newcommand{\vm}{\vec{m}}
\newcommand{\vM}{\vec{M}}
\newcommand{\vn}{\vec{n}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vP}{\vec{P}}
\newcommand{\vC}{\vec{C}}
\newcommand{\vT}{\vec{T}}
\newcommand{\vL}{\vec{L}}
\newcommand{\vgam}{\vec{\gamma}}
\newcommand{\va}{\vec{a}}
\newcommand{\vb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}
\newcommand{\vX}{\vec{X}}
\newcommand{\vY}{\vec{Y}}
\newcommand{\vZ}{\vec{Z}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vF}{\vec{F}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vV}{\mathcal{V}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vxi}{\vec{\xi}}
\newcommand{\vxb}{\vec{x}_{\textrm{b}}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vqA}{\vec{q}^{\textrm{A}}}
\newcommand{\vqB}{\vec{q}^{\textrm{B}}}
\newcommand{\vO}{\vec{0}}
\newcommand{\vS}{\vec{S}}
\newcommand{\vA}{\vec{A}}
\newcommand{\vB}{\vec{B}}
\newcommand{\bib}{\bi_{\textrm{b}}}
\newcommand{\vqa}{\vec{q}^{a}}
\newcommand{\vqb}{\vec{q}^{b}}
\newcommand{\vqc}{\vec{q}^{c}}
\newcommand{\vQ}{\vec{Q}}
\newcommand{\vQa}{\vec{Q}^{a}}
\newcommand{\vQb}{\vec{Q}^{b}}
\newcommand{\vQc}{\vec{Q}^{c}}

\newcommand{\qA}{q^{\textrm{A}}}
\newcommand{\qB}{q^{\textrm{B}}}
\newcommand{\qC}{q^{\textrm{C}}}
\newcommand{\ind}{\mathbbm{1}}
\newcommand{\ax}[2]{#1^{(#2)}}
\newcommand{\axphi}[1]{\ax{\phi}{#1}}
\newcommand{\axpsi}[1]{\ax{\psi}{#1}}
\newcommand{\axrho}[1]{\ax{\rho}{#1}}
\newcommand{\axph}[1]{\ax{p_{h}}{#1}}
\newcommand{\axp}[1]{\ax{p}{#1}}
\newcommand{\axq}[1]{\ax{q}{#1}}
\newcommand{\axf}[1]{\ax{f}{#1}}

% mesh variables
\newcommand{\laphdsym}[1]{\Delta_{#1}^{h}}
\newcommand{\laphd}[2]{\Delta_{#1}^{h}\,#2}
\newcommand{\laphdof}[3]{\paren{\laphd{#1}{#2}}_{#3}}
\newcommand{\Lhd}[2]{L_{#1}^{h}\,#2}
\newcommand{\Lhdof}[3]{\paren{\Lhd{#1}{#2}}_{#3}}
\newcommand{\mv}[2]{#1_{#2}^{h}}
\newcommand{\mvof}[3]{\paren{\mv{#1}{#2}}_{#3}}
\newcommand{\rhohd}[1]{\mv{\rho}{#1}}
\newcommand{\rhohdof}[2]{\mvof{\rho}{#1}{#2}}
\newcommand{\rhohtwodof}[2]{\big(\Lambda_{#1}^{N\from2N}\rho_{#1}^{h/2}\big)_{#2}}

\newcommand{\deltah}{\delta^{h}}
\newcommand{\deltahof}[1]{\deltah_{#1}}
\newcommand{\fhof}[3]{\paren{f_{#1}^{h}}_{#3}^{#2}}

\DeclareMathOperator{\erf}{erf}
\DeclareMathOperator{\sinc}{sinc}

\def\N{\mathbb{N}} 
\def\R{\mathbb{R}} 
\def\Q{\mathbb{Q}} 
\def\C{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\def\I{{I}}
%\def\@QC#1{\mathpalette{\setbox0=\hbox\bgr
%\def\I{{I}}
%\def\N{{\rm I\mkern-3mu N}}
%\def\R{{\rm I\mkern-3mu R}}
%\def\Q{{\@QC Q}}
%\def\C{{\@QC C}}
%\def\@QC#1{\mathpalette{\setbox0=\hbox\bgroup$\rm}%
%  {\egroup C$\egroup\rm\rlap{\kern0.4\wd0\vrule
%      width 0.05\wd0 height 0.97\ht0 depth -0.01\ht0}%
%    #1\bgroup}}
%\DeclareFontFamily{U}{cmmz}{}
%\DeclareFontShape{U}{cmmz}{m}{n}{<-8><8><9><10>%
%  <10.95><12><14.4><17.28><20.74><24.88>cmmz10}{}
%\DeclareSymbolFont{mz}{U}{cmmz}{m}{n}
%\DeclareMathSymbol\Z{\mathord}{mz}{"5A}



\newcommand{\preps}{\partial R_{\epsilon}}
\newcommand{\reps}{R_{\epsilon}}
\newcommand{\pb}{p_{\textrm{b}}}
\newcommand{\pbO}{p_{\textrm{b},0}}
\newcommand{\ub}{u_{\textrm{b}}}
\newcommand{\Tb}{T_{\textrm{bind}}}
\newcommand{\Teq}{T_{\textrm{eq}}}

%\newcommand{\equil}[1]{#1^{\textrm{eq}}}
\newcommand{\equil}[1]{\bar{#1}}
\newcommand{\peq}{\equil{p}}
\newcommand{\pbeq}{\equil{p}_{\textrm{b}}}
\newcommand{\rhoeq}{\equil{\rho}}
\newcommand{\rhobeq}{\equil{\rho}_{\textrm{b}}}

\newcommand{\rhob}{\rho_{\textrm{b}}}
\newcommand{\rhobO}{\rho_{\textrm{b},0}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\Lb}{\mathcal{L}_{\textrm{b}}}
\newcommand{\mcU}{\mathcal{U}}
\newcommand{\mcB}{\mathcal{B}}
\newcommand{\mcBp}{\mathcal{B}_{+}}
\newcommand{\mcBm}{\mathcal{B}_{-}}
\newcommand{\flt}{\tilde{f}}
\newcommand{\ult}{\tilde{u}}
\newcommand{\ublt}{\tilde{u}_{\textrm{b}}}
\newcommand{\wmin}{w_{-}}
\newcommand{\wpl}{w_{+}}
\newcommand{\lamhat}{\beta}
\newcommand{\rhat}{\hat{r}}
\newcommand{\rohat}{\rhat_0}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Rset}{\mathcal{R}}
\newcommand{\dRset}{\partial \mathcal{R}}
\newcommand{\muhat}{\hat{\mu}}
\newcommand{\Dmat}{\mathcal{D}}
\newcommand{\Dbmat}{\mathcal{D}_{\textrm{b}}}
\newcommand{\Kd}{K_{\textrm{d}}}
\newcommand{\Id}{\mathcal{I}_d}
\DeclareMathOperator\supp{supp}
\newcommand{\dB}{\partial B}
\newcommand{\Rb}{R_{\textrm{b}}}
\newcommand{\fvol}{f_{\text{v}}}
\newcommand{\fcon}{f_{\text{c}}}
\newcommand{\OD}{\Omega_{\text{free}}}
\newcommand{\OSqD}{\Omega^{2}_{\text{free}}}
\newcommand{\pvol}{p_{\text{v}}}
\newcommand{\pbvol}{p_{\textrm{b},\text{v}}}
\newcommand{\pcon}{p_{\text{c}}}
\newcommand{\pbcon}{p_{\textrm{b},\text{c}}}
\newcommand{\muvol}{\mu_{\text{v}}}
\newcommand{\mucon}{\mu_{\text{c}}}
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\ka}{k_{\text{a}}}
\newcommand{\LRho}{\bm{L}}
\newcommand{\ip}[1]{\left<#1\right>}
\newcommand{\fb}{f_{\textrm{b}}}
\newcommand{\gb}{g_{\textrm{b}}}
\newcommand{\hb}{h_{\textrm{b}}}
\newcommand{\vRho}{\vec{\mathrm{P}}}


%%%%%%%%%%%%%%%%%%%%
% added for paper with Ying
\newcommand{\Pbound}{P_{\textrm{bound}}}
\newcommand{\kp}{\kappa^{+}}
\newcommand{\km}{\kappa^{-}}
\newcommand{\Rp}{\mathcal{R}^{+}}
\newcommand{\Rm}{\mathcal{R}^{-}}
\newcommand{\diffop}{\mathcal{L}}
\newcommand{\Rph}{\mathcal{R}^{+}_h}
\newcommand{\Rmh}{\mathcal{R}^{-}_h}
\newcommand{\diffoph}{\mathcal{L}_h}
\newcommand{\pabc}{p^{(a,b,c)}}
\newcommand{\fabc}{f^{(a,b,c)}}
\newcommand{\gabc}{g^{(a,b,c)}}
\newcommand{\Fabcijk}{F_{\bi^a \bj^b \bk^c}}
\newcommand{\vVabc}{\vV_{\bi^a \bj^b \bk^c}}
\newcommand{\mup}{\beta^{+}}
\newcommand{\mum}{\beta^{-}}
\newcommand{\kpijk}{\kappa_{i j k}^{+}}
\newcommand{\kpkij}{\kappa_{k\vert i j}^{+}}
\newcommand{\kpij}{\kappa_{i j}^{+}}
\newcommand{\kmk}{\kappa_{k}^{-}}
\newcommand{\kmijk}{\kappa_{i j k}^{-}}
\newcommand{\kmkij}{\kappa_{i j \vert k}^{-}}

\newcommand{\kphat}{\hat{\kappa}_{+}}
\newcommand{\kmhat}{\hat{\kappa}_{-}}
\newcommand{\reflOp}{\mathcal{R}}

\newcommand{\kprod}{k_{\textrm{1}}}
\newcommand{\kdecay}{k_{\textrm{2}}}
\newcommand{\assok}{k}
\newcommand{\Tf}{T_\textrm{f}}

\newcommand{\Omegaf}{\Omega_{\textrm{free}}}
\newcommand{\targ}{B_{\epsilon}(\vxrb)}
\newcommand{\targbound}{\partial B_{\epsilon}(\vxrb)}
\newcommand{\phimax}{\phi_{\textrm{max}}}
\newcommand{\Pss}{P^{\textrm{ss}}}
\newcommand{\uin}{u^{\textrm{in}}}
\newcommand{\uout}{u^{\textrm{out}}}
\newcommand{\Pin}{P^{\,\textrm{in}}}
\newcommand{\Pout}{P^{\,\textrm{out}}}
\newcommand{\CO}{C_{\vec{0}}}
\newcommand{\Teuc}{\tau_{\textrm{euc}}}
\newcommand{\xt}{\tilde{x}}
\newcommand{\yt}{\tilde{y}}
\newcommand{\dBrb}{\partial\Brb}
\newcommand{\Brho}{B_{\rho}}
\newcommand{\dBrho}{\partial \Brho}
\newcommand{\dC}{\partial C}
\newcommand{\dR}{\partial R}


%%%%%%%%%%%%%%%%%%%%%
% From Kostas's latex

\newcommand{\Def}{\overset{\text{def}}{=}}


\newcommand{\KK}{K}

\newcommand{\vrho}{\varrho}
\newcommand{\eps}{\varepsilon}

\newcommand{\Borel}{\mathscr{B}}
\newcommand{\Pspace}{\mathscr{P}}
\newcommand{\BP}{\mathbb{P}}
\newcommand{\BE}{\mathbb{E}}
\newcommand{\filt}{\mathscr{F}}
\newcommand{\gilt}{\mathscr{G}}

\newcommand{\genA}{\mathcal{A}}
\newcommand{\genL}{\mathcal{L}}

\newcommand{\lb}{\left\{}
\newcommand{\rb}{\right\}}
\newcommand{\la}{\left \langle}
\newcommand{\ra}{\right\rangle}

%%%%%%%%%%%%%%%%%%%%%
% Added by Jingwei
\newcommand{\RN}[1]{% Roman Numbers in equations
  \textup{\uppercase\expandafter{\romannumeral#1}}%
}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 




